Sparse MoEs meet Efficient Ensembles

Machine learning models based on the aggregated outputs of submodels, either at the activation or prediction levels, often exhibit strong performance compared to individual models. We study the interplay of two popular classes of such models: ensembles of neural networks and sparse mixture of experts (sparse MoEs). First, we show that the two approaches have complementary features whose combination is beneficial. This includes a comprehensive evaluation of sparse MoEs in uncertainty related benchmarks. Then, we present Efficient Ensemble of Experts (E$^3$), a scalable and simple ensemble of sparse MoEs that takes the best of both classes of models, while using up to 45% fewer FLOPs than a deep ensemble. Extensive experiments demonstrate the accuracy, log-likelihood, few-shot learning, robustness, and uncertainty improvements of E$^3$ over several challenging vision Transformer-based baselines. E$^3$ not only preserves its efficiency while scaling to models with up to 2.7B parameters, but also provides better predictive performance and uncertainty estimates for larger models.

==> TMLR_rebuttal_material.tex <==

\begin{tabular}{lr}
\toprule
                           model &      GFLOPs \\
\midrule
     Last-2 k=2 m=2 o=2 (k\_up=2) &  138.457437 \\
     Last-2 k=2 m=2 o=4 (k\_up=2) &  138.457809 \\
     Last-2 k=2 m=2 o=8 (k\_up=2) &  138.458552 \\
    Last-2 k=2 m=2 o=16 (k\_up=2) &  138.459984 \\
 Last-2 k=2 partition=2 (k\_up=2) &   97.884693 \\
   Last-2 multipred k=2 (k\_up=2) &   96.330277 \\
   Last-2 multipred k=4 (k\_up=2) &  122.526318 \\
   Last-2 multipred k=8 (k\_up=2) &  175.888634 \\
    Last-2 k=2 tiling=2 (k\_up=2) &  138.459806 \\
             Last-2 k=2 (k\_up=2) &   96.895158 \\
             Last-2 k=4 (k\_up=2) &  123.644289 \\
             Last-2 k=8 (k\_up=2) &  178.132636 \\
         Last-2 k=2 m=2 (k\_up=2) &  138.457083 \\
\bottomrule
\end{tabular}


\begin{tabular}{lr}
\toprule
                           model &      GFLOPs \\
\midrule
     Last-2 k=2 m=2 o=2 (k\_up=2) &  138.457437 \\
     Last-2 k=2 m=2 o=4 (k\_up=2) &  138.457809 \\
     Last-2 k=2 m=2 o=8 (k\_up=2) &  138.458552 \\
    Last-2 k=2 m=2 o=16 (k\_up=2) &  138.459984 \\
 Last-2 k=2 partition=2 (k\_up=2) &   97.884693 \\
   Last-2 multipred k=2 (k\_up=2) &   96.330277 \\
   Last-2 multipred k=4 (k\_up=2) &  122.526318 \\
   Last-2 multipred k=8 (k\_up=2) &  175.888634 \\
    Last-2 k=2 tiling=2 (k\_up=2) &  138.459806 \\
             Last-2 k=2 (k\_up=2) &   96.895158 \\
             Last-2 k=4 (k\_up=2) &  123.644289 \\
             Last-2 k=8 (k\_up=2) &  178.132636 \\
         Last-2 k=1 m=2 (k\_up=2) &  109.781225 \\
         Last-2 k=2 m=2 (k\_up=2) &  138.457083 \\
         Last-2 k=4 m=2 (k\_up=2) &  196.869907 \\
\bottomrule
\end{tabular}









\begin{tabular}{lllrrrrr}
\toprule
                        &       &       &  val\_loss &  val\_prec\_1 &  test\_loss &  test\_prec\_1 &   test\_err \\
description & lr & total\_steps &           &             &            &              &            \\
\midrule
Last-2 k=1 m=2 (k\_up=4) & 0.005 & 30000 &  0.520872 &    0.857113 &   0.621526 &     0.831853 &  16.814667 \\
Last-2 k=1 m=4 (k\_up=4) & 0.005 & 40000 &  0.522474 &    0.856905 &   0.622106 &     0.830713 &  16.928667 \\
\bottomrule
\end{tabular}

\begin{tabular}{lllrrrrr}
\toprule
                        &       &       &  val\_loss &  val\_prec\_1 &  test\_loss &  test\_prec\_1 &  test\_err \\
description & lr & total\_steps &           &             &            &              &           \\
\midrule
Last-2 k=1 m=2 (k\_up=4) & 0.005 & 30000 &   0.00194 &    0.000972 &   0.001381 &     0.000521 &  0.052068 \\
Last-2 k=1 m=4 (k\_up=4) & 0.005 & 40000 &   0.00062 &    0.001578 &   0.000259 &     0.000158 &  0.015762 \\
\bottomrule
\end{tabular}



\begin{tabular}{llrrrrr}
\toprule
     & metric &        acc &        kl &       ece &       nll &    err \\
model\_size & model\_type &            &           &           &           &            \\
\midrule
B/32 & vmoe k=1 e=16 ens &  84.028000 &  0.211168 &  0.014570 &  0.587765 &  15.972000 \\
     & vmoe k=1 e=16 sm &  83.001999 &  0.000000 &  0.029826 &  0.640467 &  16.998002 \\
     & vmoe k=1 e=8 ens &  84.175995 &  0.228241 &  0.017342 &  0.577191 &  15.824002 \\
     & vmoe k=1 e=8 sm &  82.307999 &  0.000000 &  0.034462 &  0.660700 &  17.691998 \\
     & vmoe k=2 e=16 ens &  84.248001 &  0.211309 &  0.015688 &  0.583278 &  15.752000 \\
     & vmoe k=2 e=16 sm &  83.117996 &  0.000000 &  0.033475 &  0.637762 &  16.881999 \\
     & vmoe k=2 e=8 ens &  84.064003 &  0.183697 &  0.015335 &  0.580121 &  15.935999 \\
     & vmoe k=2 e=8 sm &  82.520004 &  0.000000 &  0.025071 &  0.649235 &  17.479999 \\
\bottomrule
\end{tabular}

\begin{tabular}{llrrrrr}
\toprule
     & metric &       acc &   kl &       ece &       nll &   acc/err \\
model\_size & model\_type &           &      &           &           &           \\
\midrule
B/32 & vmoe k=1 e=16 ens &       NaN &  NaN &       NaN &       NaN &       NaN \\
     & vmoe k=1 e=16 sm &  0.112000 &  0.0 &  0.000105 &  0.006406 &  0.112000 \\
     & vmoe k=1 e=8 ens &       NaN &  NaN &       NaN &       NaN &       NaN \\
     & vmoe k=1 e=8 sm &  0.082941 &  0.0 &  0.000430 &  0.003393 &  0.082941 \\
     & vmoe k=2 e=16 ens &       NaN &  NaN &       NaN &       NaN &       NaN \\
     & vmoe k=2 e=16 sm &  0.086002 &  0.0 &  0.000940 &  0.006644 &  0.086001 \\
     & vmoe k=2 e=8 ens &       NaN &  NaN &       NaN &       NaN &       NaN \\
     & vmoe k=2 e=8 sm &  0.095872 &  0.0 &  0.000314 &  0.002115 &  0.095872 \\
\bottomrule
\end{tabular}



\begin{tabular}{lrrr}
\toprule
{} &  test\_loss &  test\_prec\_1 &  test\_err \\
description             &            &              &           \\
\midrule
Last-2 k=1 m=2 (k\_up=2) &   0.620492 &     0.832020 &   16.7980 \\
Last-2 k=2 m=2 (k\_up=2) &   0.608367 &     0.835328 &   16.4672 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrr}
\toprule
{} &  test\_loss &  test\_prec\_1 &  test\_err \\
description             &            &              &           \\
\midrule
Last-2 k=1 m=2 (k\_up=2) &   0.000831 &     0.000395 &  0.039532 \\
Last-2 k=2 m=2 (k\_up=2) &   0.000171 &     0.000331 &  0.033091 \\
\bottomrule
\end{tabular}

==> new_FLOPs_table.tex <==
\begin{table}[h]
\centering
\begin{tabular}{c|cc|cccccc}
\toprule
{} &  K &  M &    S/32 &    B/32 &     B/16 &     L/32 &     L/16 &      H/14 \\
\midrule
E$^3$ &  1 &  2 &   36.69 &  105.89 &   452.62 &   320.92 &  1356.46 &   4183.28 \\
E$^3$ &  1 &  4 &   58.03 &  152.98 &      ---    &   403.77 &      ---    &       ---    \\
E$^3$ &  2 &  2 &   47.98 &  131.06 &   552.65 &   365.42 &  1533.74 &       ---    \\
E$^3$ &  2 &  4 &   80.66 &  203.31 &      ---    &   492.77 &      ---    &       ---    \\
E$^3$ &  4 &  2 &   70.61 &  181.40 &      ---    &   454.43 &      ---    &       ---    \\
ViT   &  - &  1 &   24.01 &   77.97 &   334.48 &   271.83 &  1151.71 &   3033.60 \\
ViT   &  - &  2 &   48.02 &  155.93 &   668.95 &   543.66 &  2303.43 &   6067.21 \\
ViT   &  - &  4 &   96.03 &  311.87 &  1337.90 &  1087.33 &  4606.85 &  12134.41 \\
V-MoE &  1 &  1 &   26.02 &   82.35 &   351.91 &   279.55 &  1182.08 &   3179.90 \\
V-MoE &  1 &  2 &   52.04 &  164.70 &   703.81 &   559.10 &  2364.16 &   6359.81 \\
V-MoE &  1 &  4 &  104.07 &  329.41 &  1407.63 &  1118.21 &  4728.32 &  12719.61 \\
V-MoE &  2 &  1 &   31.66 &   94.93 &   401.98 &   301.75 &  1270.78 &   3617.94 \\
V-MoE &  4 &  1 &   42.95 &  120.11 &   501.99 &   346.25 &  1448.06 &       ---    \\
V-MoE &  8 &  1 &   65.59 &  170.44 &      ---    &   435.26 &      ---    &       ---    \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{c|cccccc}
\toprule
{} &    S/32 &    B/32 &    B/16 &    L/32 &    L/16 &    H/14 \\
\midrule
E$^3$ (1, 2) vs. V-MoE (1)    &   41.01 &   28.58 &   28.62 &   14.80 &   14.75 &   31.55 \\
E$^3$ (1, 2) vs. V-MoE (1, 2) &  -29.49 &  -35.71 &  -35.69 &  -42.60 &  -42.62 &  -34.22 \\
\bottomrule
\end{tabular}
\end{table}

==> new_efficient_ensemble_table.tex <==
\begin{tabular}{cccccccc}
\toprule
 & \textsc{K} & \textsc{M} &                      \textsc{NLL} &                   \textsc{Error} &                      \textsc{ECE} &                       \textsc{KL} & \textsc{GFLOPs} \\
\midrule
ViT &         -- &         -- &  0.688 {\tiny \color{gray} $\pm$ 0.003} &  18.65 {\tiny \color{gray} $\pm$ 0.08} &  0.022 {\tiny \color{gray} $\pm$ 0.000} &                                -- &            78.0 \\
\cmidrule{1-8}
\multirow{2}{*}{BE ViT} &         -- &          2 &  0.682 {\tiny \color{gray} $\pm$ 0.003} &  18.47 {\tiny \color{gray} $\pm$ 0.05} &  0.021 {\tiny \color{gray} $\pm$ 0.000} &  0.040 {\tiny \color{gray} $\pm$ 0.001} &            97.1 \\
 &         -- &          4 &  0.675 {\tiny \color{gray} $\pm$ 0.003} &  18.40 {\tiny \color{gray} $\pm$ 0.09} &  0.017 {\tiny \color{gray} $\pm$ 0.000} &  0.035 {\tiny \color{gray} $\pm$ 0.001} &           135.4 \\
\cmidrule{1-8}
\multirow{4}{*}{V-MoE} &          1 &         -- &  0.642 {\tiny \color{gray} $\pm$ 0.002} &  16.90 {\tiny \color{gray} $\pm$ 0.05} &  0.029 {\tiny \color{gray} $\pm$ 0.001} &                                -- &            82.4 \\
 &          2 &         -- &  0.638 {\tiny \color{gray} $\pm$ 0.001} &  16.76 {\tiny \color{gray} $\pm$ 0.05} &  0.033 {\tiny \color{gray} $\pm$ 0.001} &                                -- &            94.9 \\
 &          4 &         -- &  0.636 {\tiny \color{gray} $\pm$ 0.001} &  16.70 {\tiny \color{gray} $\pm$ 0.04} &  0.034 {\tiny \color{gray} $\pm$ 0.001} &                                -- &           120.1 \\
 &          8 &         -- &  0.635 {\tiny \color{gray} $\pm$ 0.002} &  16.72 {\tiny \color{gray} $\pm$ 0.06} &  0.028 {\tiny \color{gray} $\pm$ 0.001} &                                -- &           170.4 \\
\cmidrule{1-8}
\multirow{5}{*}{MC dropout V-MoE} &          1 &          2 &  0.648 {\tiny \color{gray} $\pm$ 0.002} &  17.10 {\tiny \color{gray} $\pm$ 0.05} &  0.019 {\tiny \color{gray} $\pm$ 0.001} &  0.046 {\tiny \color{gray} $\pm$ 0.000} &            97.2 \\
 &          1 &          4 &  0.641 {\tiny \color{gray} $\pm$ 0.002} &  16.96 {\tiny \color{gray} $\pm$ 0.05} &  0.017 {\tiny \color{gray} $\pm$ 0.001} &  0.046 {\tiny \color{gray} $\pm$ 0.001} &           135.6 \\
 &          2 &          2 &  0.642 {\tiny \color{gray} $\pm$ 0.002} &  16.94 {\tiny \color{gray} $\pm$ 0.04} &  0.021 {\tiny \color{gray} $\pm$ 0.001} &  0.046 {\tiny \color{gray} $\pm$ 0.001} &           113.7 \\
 &          2 &          4 &  0.634 {\tiny \color{gray} $\pm$ 0.001} &  16.80 {\tiny \color{gray} $\pm$ 0.03} &  0.020 {\tiny \color{gray} $\pm$ 0.000} &  0.046 {\tiny \color{gray} $\pm$ 0.001} &           168.6 \\
 &          4 &          2 &  0.639 {\tiny \color{gray} $\pm$ 0.002} &  16.91 {\tiny \color{gray} $\pm$ 0.06} &  0.022 {\tiny \color{gray} $\pm$ 0.001} &  0.045 {\tiny \color{gray} $\pm$ 0.001} &           146.7 \\
\cmidrule{1-8}
\multirow{2}{*}{MIMO V-MoE (BR=1)} &          2 &          2 &  0.636 {\tiny \color{gray} $\pm$ 0.002} &  16.97 {\tiny \color{gray} $\pm$ 0.04} &  0.028 {\tiny \color{gray} $\pm$ 0.001} &  0.000 {\tiny \color{gray} $\pm$ 0.000} &            96.3 \\
 &          2 &          4 &  0.672 {\tiny \color{gray} $\pm$ 0.001} &  17.72 {\tiny \color{gray} $\pm$ 0.04} &  0.037 {\tiny \color{gray} $\pm$ 0.000} &  0.001 {\tiny \color{gray} $\pm$ 0.000} &            99.0 \\
\multirow{2}{*}{MIMO V-MoE (BR=2)} &          2 &          2 &  0.638 {\tiny \color{gray} $\pm$ 0.001} &  17.14 {\tiny \color{gray} $\pm$ 0.03} &  0.031 {\tiny \color{gray} $\pm$ 0.000} &  0.001 {\tiny \color{gray} $\pm$ 0.000} &           192.6 \\
 &          2 &          4 &  0.665 {\tiny \color{gray} $\pm$ 0.002} &  17.38 {\tiny \color{gray} $\pm$ 0.04} &  0.038 {\tiny \color{gray} $\pm$ 0.000} &  0.000 {\tiny \color{gray} $\pm$ 0.000} &           198.1 \\
\cmidrule{1-8}
\multirow{5}{*}{\ack} &          1 &          2 &  0.622 {\tiny \color{gray} $\pm$ 0.001} &  16.70 {\tiny \color{gray} $\pm$ 0.03} &  0.018 {\tiny \color{gray} $\pm$ 0.000} &  0.217 {\tiny \color{gray} $\pm$ 0.003} &           105.9 \\
 &          1 &          4 &  0.624 {\tiny \color{gray} $\pm$ 0.001} &  16.99 {\tiny \color{gray} $\pm$ 0.03} &  0.013 {\tiny \color{gray} $\pm$ 0.000} &  0.164 {\tiny \color{gray} $\pm$ 0.001} &           153.0 \\
 &          2 &          2 &  0.612 {\tiny \color{gray} $\pm$ 0.001} &  16.49 {\tiny \color{gray} $\pm$ 0.02} &  0.013 {\tiny \color{gray} $\pm$ 0.000} &  0.198 {\tiny \color{gray} $\pm$ 0.003} &           131.1 \\
 &          2 &          4 &  0.620 {\tiny \color{gray} $\pm$ 0.001} &  16.86 {\tiny \color{gray} $\pm$ 0.02} &  0.015 {\tiny \color{gray} $\pm$ 0.000} &  0.170 {\tiny \color{gray} $\pm$ 0.001} &           203.3 \\
 &          4 &          2 &  0.611 {\tiny \color{gray} $\pm$ 0.001} &  16.45 {\tiny \color{gray} $\pm$ 0.03} &  0.014 {\tiny \color{gray} $\pm$ 0.000} &  0.193 {\tiny \color{gray} $\pm$ 0.003} &           181.4 \\
\bottomrule
\end{tabular}


==> new_tables_with_delta_FLOPs.tex <==
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc|cccc|cccc|c}
\toprule
     &       & \multicolumn{2}{c}{\;} & \multicolumn{4}{c}{\textsc{Mean Across Datasets}} & \multicolumn{4}{c}{\textsc{Weighted Mean Across Datasets}} &                      \textsc{Downstream} \\
     &       & \textsc{K} & \textsc{M} &              \textsc{1-Shot Error} $\downarrow$ &              \textsc{5-Shot Error} $\downarrow$ &             \textsc{10-Shot Error} $\downarrow$ &             \textsc{25-Shot Error} $\downarrow$ &              \textsc{1-Shot Error} $\downarrow$ &              \textsc{5-Shot Error} $\downarrow$ &             \textsc{10-Shot Error} $\downarrow$ &             \textsc{25-Shot Error} $\downarrow$ & $\Delta$\textsc{FLOPs} (\%) $\downarrow$ \\
\midrule
\multirow{3}{*}{H/14} & E$^3$ &          1 &          2 &  \textbf{31.47} {\tiny \color{gray} $\pm$ 0.72} &  \textbf{17.87} {\tiny \color{gray} $\pm$ 0.32} &  \textbf{14.29} {\tiny \color{gray} $\pm$ 0.22} &  \textbf{10.64} {\tiny \color{gray} $\pm$ 0.25} &  \textbf{78.51} {\tiny \color{gray} $\pm$ 0.24} &  \textbf{80.65} {\tiny \color{gray} $\pm$ 0.08} &  \textbf{81.28} {\tiny \color{gray} $\pm$ 0.05} &  \textbf{81.51} {\tiny \color{gray} $\pm$ 0.06} &                           \textbf{15.63} \\
     & down-DE &          1 &          2 &  \textbf{30.84} {\tiny \color{gray} $\pm$ 0.42} &  \textbf{17.77} {\tiny \color{gray} $\pm$ 0.51} &  \textbf{14.43} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{11.06} {\tiny \color{gray} $\pm$ 0.40} &  \textbf{78.36} {\tiny \color{gray} $\pm$ 0.20} &  \textbf{80.63} {\tiny \color{gray} $\pm$ 0.14} &  \textbf{81.31} {\tiny \color{gray} $\pm$ 0.02} &  \textbf{81.60} {\tiny \color{gray} $\pm$ 0.09} &                                    75.79 \\
     & V-MoE &          2 &          1 &  \textbf{32.47} {\tiny \color{gray} $\pm$ 0.55} &  \textbf{18.77} {\tiny \color{gray} $\pm$ 0.41} &           15.19 {\tiny \color{gray} $\pm$ 0.27} &           12.09 {\tiny \color{gray} $\pm$ 0.38} &  \textbf{78.93} {\tiny \color{gray} $\pm$ 0.20} &  \textbf{80.89} {\tiny \color{gray} $\pm$ 0.11} &           81.48 {\tiny \color{gray} $\pm$ 0.07} &           81.83 {\tiny \color{gray} $\pm$ 0.09} &                                      --- \\
\cmidrule{1-13}
\multirow{3}{*}{L/16} & E$^3$ &          1 &          2 &  \textbf{34.08} {\tiny \color{gray} $\pm$ 0.21} &  \textbf{19.57} {\tiny \color{gray} $\pm$ 0.16} &  \textbf{15.21} {\tiny \color{gray} $\pm$ 0.14} &  \textbf{11.75} {\tiny \color{gray} $\pm$ 0.11} &           79.50 {\tiny \color{gray} $\pm$ 0.07} &  \textbf{81.09} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{81.48} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{81.76} {\tiny \color{gray} $\pm$ 0.02} &                            \textbf{6.74} \\
     & down-DE &          1 &          2 &  \textbf{32.98} {\tiny \color{gray} $\pm$ 0.42} &  \textbf{19.65} {\tiny \color{gray} $\pm$ 0.16} &  \textbf{15.44} {\tiny \color{gray} $\pm$ 0.16} &  \textbf{11.92} {\tiny \color{gray} $\pm$ 0.14} &  \textbf{79.09} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{81.10} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{81.54} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{81.79} {\tiny \color{gray} $\pm$ 0.03} &                                    86.04 \\
     & V-MoE &          2 &          1 &  \textbf{33.98} {\tiny \color{gray} $\pm$ 0.28} &           20.42 {\tiny \color{gray} $\pm$ 0.12} &           16.20 {\tiny \color{gray} $\pm$ 0.08} &           12.73 {\tiny \color{gray} $\pm$ 0.13} &  \textbf{79.50} {\tiny \color{gray} $\pm$ 0.10} &           81.30 {\tiny \color{gray} $\pm$ 0.03} &           81.72 {\tiny \color{gray} $\pm$ 0.02} &           81.97 {\tiny \color{gray} $\pm$ 0.03} &                                      --- \\
\cmidrule{1-13}
\multirow{3}{*}{L/32} & E$^3$ &          1 &          2 &  \textbf{36.71} {\tiny \color{gray} $\pm$ 0.20} &  \textbf{22.14} {\tiny \color{gray} $\pm$ 0.16} &  \textbf{17.79} {\tiny \color{gray} $\pm$ 0.05} &  \textbf{13.97} {\tiny \color{gray} $\pm$ 0.09} &  \textbf{80.51} {\tiny \color{gray} $\pm$ 0.07} &  \textbf{81.77} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{82.11} {\tiny \color{gray} $\pm$ 0.01} &  \textbf{82.26} {\tiny \color{gray} $\pm$ 0.02} &                            \textbf{6.35} \\
     & down-DE &          1 &          2 &  \textbf{36.15} {\tiny \color{gray} $\pm$ 0.28} &  \textbf{22.18} {\tiny \color{gray} $\pm$ 0.15} &  \textbf{17.81} {\tiny \color{gray} $\pm$ 0.14} &  \textbf{14.00} {\tiny \color{gray} $\pm$ 0.12} &  \textbf{80.45} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{81.79} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{82.13} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{82.27} {\tiny \color{gray} $\pm$ 0.03} &                                    85.29 \\
     & V-MoE &          2 &          1 &  \textbf{36.56} {\tiny \color{gray} $\pm$ 0.34} &           23.00 {\tiny \color{gray} $\pm$ 0.12} &           18.86 {\tiny \color{gray} $\pm$ 0.07} &           15.02 {\tiny \color{gray} $\pm$ 0.16} &  \textbf{80.56} {\tiny \color{gray} $\pm$ 0.13} &           82.00 {\tiny \color{gray} $\pm$ 0.03} &           82.37 {\tiny \color{gray} $\pm$ 0.02} &           82.50 {\tiny \color{gray} $\pm$ 0.03} &                                      --- \\
\cmidrule{1-13}
\multirow{3}{*}{B/16} & E$^3$ &          1 &          2 &  \textbf{38.60} {\tiny \color{gray} $\pm$ 0.38} &  \textbf{21.93} {\tiny \color{gray} $\pm$ 0.17} &  \textbf{17.43} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{13.62} {\tiny \color{gray} $\pm$ 0.08} &  \textbf{81.14} {\tiny \color{gray} $\pm$ 0.11} &  \textbf{81.74} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{82.05} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{82.19} {\tiny \color{gray} $\pm$ 0.02} &                           \textbf{12.60} \\
     & down-DE &          1 &          2 &           38.96 {\tiny \color{gray} $\pm$ 0.36} &           23.36 {\tiny \color{gray} $\pm$ 0.23} &           18.99 {\tiny \color{gray} $\pm$ 0.12} &           14.84 {\tiny \color{gray} $\pm$ 0.11} &           81.39 {\tiny \color{gray} $\pm$ 0.10} &           82.09 {\tiny \color{gray} $\pm$ 0.06} &           82.40 {\tiny \color{gray} $\pm$ 0.03} &           82.46 {\tiny \color{gray} $\pm$ 0.02} &                                    75.09 \\
     & V-MoE &          2 &          1 &  \textbf{37.76} {\tiny \color{gray} $\pm$ 0.15} &           23.16 {\tiny \color{gray} $\pm$ 0.09} &           18.79 {\tiny \color{gray} $\pm$ 0.14} &           14.94 {\tiny \color{gray} $\pm$ 0.16} &  \textbf{80.97} {\tiny \color{gray} $\pm$ 0.05} &           82.04 {\tiny \color{gray} $\pm$ 0.02} &           82.36 {\tiny \color{gray} $\pm$ 0.03} &           82.48 {\tiny \color{gray} $\pm$ 0.04} &                                      --- \\
\cmidrule{1-13}
\multirow{3}{*}{B/32} & E$^3$ &          1 &          2 &           43.39 {\tiny \color{gray} $\pm$ 0.33} &  \textbf{26.51} {\tiny \color{gray} $\pm$ 0.11} &  \textbf{21.18} {\tiny \color{gray} $\pm$ 0.17} &  \textbf{16.82} {\tiny \color{gray} $\pm$ 0.09} &           82.86 {\tiny \color{gray} $\pm$ 0.11} &  \textbf{82.91} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{82.93} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{82.90} {\tiny \color{gray} $\pm$ 0.02} &                           \textbf{11.54} \\
     & down-DE &          1 &          2 &  \textbf{41.09} {\tiny \color{gray} $\pm$ 0.31} &  \textbf{26.48} {\tiny \color{gray} $\pm$ 0.24} &  \textbf{21.61} {\tiny \color{gray} $\pm$ 0.22} &  \textbf{17.20} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{82.24} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{82.89} {\tiny \color{gray} $\pm$ 0.06} &  \textbf{83.03} {\tiny \color{gray} $\pm$ 0.05} &  \textbf{82.99} {\tiny \color{gray} $\pm$ 0.03} &                                    73.49 \\
     & V-MoE &          2 &          1 &           42.50 {\tiny \color{gray} $\pm$ 0.28} &           27.44 {\tiny \color{gray} $\pm$ 0.19} &           22.73 {\tiny \color{gray} $\pm$ 0.19} &           18.60 {\tiny \color{gray} $\pm$ 0.19} &           82.66 {\tiny \color{gray} $\pm$ 0.08} &           83.16 {\tiny \color{gray} $\pm$ 0.05} &           83.29 {\tiny \color{gray} $\pm$ 0.05} &           83.29 {\tiny \color{gray} $\pm$ 0.04} &                                      --- \\
\cmidrule{1-13}
\multirow{3}{*}{S/32} & E$^3$ &          1 &          2 &           52.91 {\tiny \color{gray} $\pm$ 0.27} &           34.28 {\tiny \color{gray} $\pm$ 0.19} &           27.54 {\tiny \color{gray} $\pm$ 0.18} &  \textbf{21.85} {\tiny \color{gray} $\pm$ 0.11} &           85.89 {\tiny \color{gray} $\pm$ 0.08} &           84.81 {\tiny \color{gray} $\pm$ 0.04} &           84.39 {\tiny \color{gray} $\pm$ 0.04} &  \textbf{84.01} {\tiny \color{gray} $\pm$ 0.02} &                           \textbf{15.87} \\
     & down-DE &          1 &          2 &  \textbf{48.27} {\tiny \color{gray} $\pm$ 0.21} &  \textbf{32.19} {\tiny \color{gray} $\pm$ 0.22} &  \textbf{26.55} {\tiny \color{gray} $\pm$ 0.10} &  \textbf{21.95} {\tiny \color{gray} $\pm$ 0.20} &  \textbf{84.62} {\tiny \color{gray} $\pm$ 0.06} &  \textbf{84.35} {\tiny \color{gray} $\pm$ 0.05} &  \textbf{84.19} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{84.04} {\tiny \color{gray} $\pm$ 0.05} &                                    64.34 \\
     & V-MoE &          2 &          1 &           49.37 {\tiny \color{gray} $\pm$ 0.19} &           33.51 {\tiny \color{gray} $\pm$ 0.17} &           28.00 {\tiny \color{gray} $\pm$ 0.14} &           23.25 {\tiny \color{gray} $\pm$ 0.15} &           85.04 {\tiny \color{gray} $\pm$ 0.06} &           84.69 {\tiny \color{gray} $\pm$ 0.04} &           84.54 {\tiny \color{gray} $\pm$ 0.03} &           84.33 {\tiny \color{gray} $\pm$ 0.03} &                                      --- \\
\bottomrule
\end{tabular}
}


\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc|ccc|ccc|ccc|ccc|c}
\toprule
     &       & \multicolumn{2}{c}{\;} & \multicolumn{3}{c}{\textsc{ImageNet}} & \multicolumn{3}{c}{\textsc{ImageNet-C (average)}} & \multicolumn{3}{c}{\textsc{ImageNet-A}} & \multicolumn{3}{c}{\textsc{ImageNet-V2}} &                      \textsc{Downstream} \\
     &       & \textsc{K} & \textsc{M} &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ & $\Delta$\textsc{FLOPs} (\%) $\downarrow$ \\
\midrule
\multirow{3}{*}{H/14} & E$^3$ &          1 &          2 &           0.408 {\tiny \color{gray} $\pm$ 0.001} &           11.63 {\tiny \color{gray} $\pm$ 0.05} &  \textbf{0.012} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.865} {\tiny \color{gray} $\pm$ 0.010} &  \textbf{21.46} {\tiny \color{gray} $\pm$ 0.16} &  \textbf{0.018} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{2.276} {\tiny \color{gray} $\pm$ 0.042} &  \textbf{49.09} {\tiny \color{gray} $\pm$ 0.78} &  \textbf{0.101} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{0.745} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{19.50} {\tiny \color{gray} $\pm$ 0.08} &  \textbf{0.035} {\tiny \color{gray} $\pm$ 0.001} &                           \textbf{15.63} \\
     & down-DE &          1 &          2 &  \textbf{0.403} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{11.35} {\tiny \color{gray} $\pm$ 0.05} &           0.018 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.871} {\tiny \color{gray} $\pm$ 0.012} &  \textbf{21.37} {\tiny \color{gray} $\pm$ 0.20} &           0.021 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{2.273} {\tiny \color{gray} $\pm$ 0.049} &  \textbf{47.93} {\tiny \color{gray} $\pm$ 0.93} &  \textbf{0.108} {\tiny \color{gray} $\pm$ 0.001} &           0.758 {\tiny \color{gray} $\pm$ 0.003} &  \textbf{19.28} {\tiny \color{gray} $\pm$ 0.17} &           0.044 {\tiny \color{gray} $\pm$ 0.001} &                                    75.79 \\
     & V-MoE &          2 &          1 &           0.428 {\tiny \color{gray} $\pm$ 0.003} &           11.89 {\tiny \color{gray} $\pm$ 0.13} &           0.030 {\tiny \color{gray} $\pm$ 0.001} &           0.934 {\tiny \color{gray} $\pm$ 0.013} &           22.41 {\tiny \color{gray} $\pm$ 0.20} &           0.038 {\tiny \color{gray} $\pm$ 0.001} &           2.517 {\tiny \color{gray} $\pm$ 0.063} &  \textbf{50.34} {\tiny \color{gray} $\pm$ 1.12} &           0.167 {\tiny \color{gray} $\pm$ 0.003} &           0.811 {\tiny \color{gray} $\pm$ 0.005} &           20.25 {\tiny \color{gray} $\pm$ 0.13} &           0.065 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{L/16} & E$^3$ &          1 &          2 &  \textbf{0.448} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{12.60} {\tiny \color{gray} $\pm$ 0.03} &           0.020 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.023} {\tiny \color{gray} $\pm$ 0.005} &  \textbf{24.89} {\tiny \color{gray} $\pm$ 0.11} &           0.024 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{2.836} {\tiny \color{gray} $\pm$ 0.015} &  \textbf{57.97} {\tiny \color{gray} $\pm$ 0.21} &           0.160 {\tiny \color{gray} $\pm$ 0.001} &           0.838 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{21.30} {\tiny \color{gray} $\pm$ 0.07} &           0.051 {\tiny \color{gray} $\pm$ 0.001} &                            \textbf{6.74} \\
     & down-DE &          1 &          2 &  \textbf{0.450} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{12.62} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.016} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.010} {\tiny \color{gray} $\pm$ 0.006} &  \textbf{24.43} {\tiny \color{gray} $\pm$ 0.12} &  \textbf{0.021} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{2.796} {\tiny \color{gray} $\pm$ 0.016} &  \textbf{57.06} {\tiny \color{gray} $\pm$ 0.32} &  \textbf{0.136} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.818} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{21.06} {\tiny \color{gray} $\pm$ 0.11} &  \textbf{0.044} {\tiny \color{gray} $\pm$ 0.001} &                                    86.04 \\
     & V-MoE &          2 &          1 &           0.464 {\tiny \color{gray} $\pm$ 0.001} &           12.88 {\tiny \color{gray} $\pm$ 0.04} &           0.025 {\tiny \color{gray} $\pm$ 0.000} &           1.058 {\tiny \color{gray} $\pm$ 0.004} &           25.27 {\tiny \color{gray} $\pm$ 0.08} &           0.034 {\tiny \color{gray} $\pm$ 0.000} &           2.945 {\tiny \color{gray} $\pm$ 0.016} &  \textbf{57.85} {\tiny \color{gray} $\pm$ 0.28} &           0.178 {\tiny \color{gray} $\pm$ 0.001} &           0.848 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{21.33} {\tiny \color{gray} $\pm$ 0.03} &           0.057 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{L/32} & E$^3$ &          1 &          2 &  \textbf{0.535} {\tiny \color{gray} $\pm$ 0.001} &           14.70 {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.027} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.193} {\tiny \color{gray} $\pm$ 0.003} &           28.28 {\tiny \color{gray} $\pm$ 0.05} &           0.032 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{4.170} {\tiny \color{gray} $\pm$ 0.010} &  \textbf{74.73} {\tiny \color{gray} $\pm$ 0.09} &           0.266 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{0.989} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{24.62} {\tiny \color{gray} $\pm$ 0.08} &  \textbf{0.063} {\tiny \color{gray} $\pm$ 0.001} &                            \textbf{6.35} \\
     & down-DE &          1 &          2 &  \textbf{0.533} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{14.55} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.025} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.184} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{27.98} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.029} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{4.139} {\tiny \color{gray} $\pm$ 0.017} &  \textbf{74.29} {\tiny \color{gray} $\pm$ 0.21} &  \textbf{0.254} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{0.982} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{24.42} {\tiny \color{gray} $\pm$ 0.08} &  \textbf{0.061} {\tiny \color{gray} $\pm$ 0.002} &                                    85.29 \\
     & V-MoE &          2 &          1 &           0.563 {\tiny \color{gray} $\pm$ 0.001} &           15.05 {\tiny \color{gray} $\pm$ 0.03} &           0.039 {\tiny \color{gray} $\pm$ 0.000} &           1.261 {\tiny \color{gray} $\pm$ 0.005} &           29.12 {\tiny \color{gray} $\pm$ 0.07} &           0.052 {\tiny \color{gray} $\pm$ 0.000} &           4.394 {\tiny \color{gray} $\pm$ 0.014} &           75.39 {\tiny \color{gray} $\pm$ 0.17} &           0.301 {\tiny \color{gray} $\pm$ 0.002} &           1.046 {\tiny \color{gray} $\pm$ 0.002} &           25.22 {\tiny \color{gray} $\pm$ 0.06} &           0.083 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{B/16} & E$^3$ &          1 &          2 &  \textbf{0.519} {\tiny \color{gray} $\pm$ 0.001} &           14.26 {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.020} {\tiny \color{gray} $\pm$ 0.000} &           1.352 {\tiny \color{gray} $\pm$ 0.005} &           31.20 {\tiny \color{gray} $\pm$ 0.09} &  \textbf{0.022} {\tiny \color{gray} $\pm$ 0.000} &           3.835 {\tiny \color{gray} $\pm$ 0.019} &           72.25 {\tiny \color{gray} $\pm$ 0.22} &           0.223 {\tiny \color{gray} $\pm$ 0.002} &           0.974 {\tiny \color{gray} $\pm$ 0.002} &           24.10 {\tiny \color{gray} $\pm$ 0.10} &  \textbf{0.051} {\tiny \color{gray} $\pm$ 0.001} &                           \textbf{12.60} \\
     & down-DE &          1 &          2 &  \textbf{0.519} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{14.09} {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.021} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.316} {\tiny \color{gray} $\pm$ 0.008} &  \textbf{30.02} {\tiny \color{gray} $\pm$ 0.18} &           0.030 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{3.618} {\tiny \color{gray} $\pm$ 0.013} &  \textbf{66.99} {\tiny \color{gray} $\pm$ 0.28} &  \textbf{0.203} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{0.945} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{23.39} {\tiny \color{gray} $\pm$ 0.09} &  \textbf{0.054} {\tiny \color{gray} $\pm$ 0.001} &                                    75.09 \\
     & V-MoE &          2 &          1 &           0.533 {\tiny \color{gray} $\pm$ 0.001} &           14.60 {\tiny \color{gray} $\pm$ 0.04} &           0.022 {\tiny \color{gray} $\pm$ 0.000} &           1.372 {\tiny \color{gray} $\pm$ 0.005} &           31.27 {\tiny \color{gray} $\pm$ 0.11} &           0.034 {\tiny \color{gray} $\pm$ 0.000} &           3.875 {\tiny \color{gray} $\pm$ 0.016} &           70.79 {\tiny \color{gray} $\pm$ 0.30} &           0.235 {\tiny \color{gray} $\pm$ 0.002} &           0.959 {\tiny \color{gray} $\pm$ 0.003} &           24.09 {\tiny \color{gray} $\pm$ 0.11} &           0.056 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{B/32} & E$^3$ &          1 &          2 &  \textbf{0.622} {\tiny \color{gray} $\pm$ 0.001} &           16.70 {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.018} {\tiny \color{gray} $\pm$ 0.000} &           1.532 {\tiny \color{gray} $\pm$ 0.005} &           34.73 {\tiny \color{gray} $\pm$ 0.08} &  \textbf{0.022} {\tiny \color{gray} $\pm$ 0.000} &           5.080 {\tiny \color{gray} $\pm$ 0.013} &           84.91 {\tiny \color{gray} $\pm$ 0.09} &           0.301 {\tiny \color{gray} $\pm$ 0.001} &           1.143 {\tiny \color{gray} $\pm$ 0.002} &           27.97 {\tiny \color{gray} $\pm$ 0.10} &  \textbf{0.055} {\tiny \color{gray} $\pm$ 0.001} &                           \textbf{11.54} \\
     & down-DE &          1 &          2 &  \textbf{0.620} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{16.44} {\tiny \color{gray} $\pm$ 0.04} &           0.023 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.510} {\tiny \color{gray} $\pm$ 0.005} &  \textbf{33.79} {\tiny \color{gray} $\pm$ 0.08} &           0.032 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{4.891} {\tiny \color{gray} $\pm$ 0.014} &  \textbf{81.98} {\tiny \color{gray} $\pm$ 0.18} &  \textbf{0.284} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{1.116} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{27.24} {\tiny \color{gray} $\pm$ 0.08} &           0.061 {\tiny \color{gray} $\pm$ 0.000} &                                    73.49 \\
     & V-MoE &          2 &          1 &           0.638 {\tiny \color{gray} $\pm$ 0.001} &           16.76 {\tiny \color{gray} $\pm$ 0.05} &           0.033 {\tiny \color{gray} $\pm$ 0.001} &           1.562 {\tiny \color{gray} $\pm$ 0.004} &           34.40 {\tiny \color{gray} $\pm$ 0.06} &           0.050 {\tiny \color{gray} $\pm$ 0.001} &           5.032 {\tiny \color{gray} $\pm$ 0.014} &  \textbf{81.71} {\tiny \color{gray} $\pm$ 0.11} &           0.317 {\tiny \color{gray} $\pm$ 0.002} &           1.150 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{27.50} {\tiny \color{gray} $\pm$ 0.08} &           0.076 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{S/32} & E$^3$ &          1 &          2 &  \textbf{0.818} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{21.18} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.015} {\tiny \color{gray} $\pm$ 0.000} &           2.169 {\tiny \color{gray} $\pm$ 0.008} &           45.79 {\tiny \color{gray} $\pm$ 0.10} &  \textbf{0.030} {\tiny \color{gray} $\pm$ 0.000} &           6.419 {\tiny \color{gray} $\pm$ 0.011} &           93.98 {\tiny \color{gray} $\pm$ 0.09} &           0.345 {\tiny \color{gray} $\pm$ 0.001} &           1.437 {\tiny \color{gray} $\pm$ 0.002} &           34.03 {\tiny \color{gray} $\pm$ 0.05} &  \textbf{0.054} {\tiny \color{gray} $\pm$ 0.001} &                           \textbf{15.87} \\
     & down-DE &          1 &          2 &  \textbf{0.807} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{20.90} {\tiny \color{gray} $\pm$ 0.10} &           0.018 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{2.106} {\tiny \color{gray} $\pm$ 0.010} &  \textbf{44.52} {\tiny \color{gray} $\pm$ 0.18} &           0.038 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{6.063} {\tiny \color{gray} $\pm$ 0.007} &  \textbf{92.33} {\tiny \color{gray} $\pm$ 0.07} &  \textbf{0.335} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.393} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{33.29} {\tiny \color{gray} $\pm$ 0.10} &           0.062 {\tiny \color{gray} $\pm$ 0.002} &                                    64.34 \\
     & V-MoE &          2 &          1 &           0.829 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{21.09} {\tiny \color{gray} $\pm$ 0.08} &           0.035 {\tiny \color{gray} $\pm$ 0.001} &           2.162 {\tiny \color{gray} $\pm$ 0.007} &  \textbf{44.95} {\tiny \color{gray} $\pm$ 0.12} &           0.066 {\tiny \color{gray} $\pm$ 0.001} &           6.227 {\tiny \color{gray} $\pm$ 0.015} &  \textbf{92.09} {\tiny \color{gray} $\pm$ 0.12} &           0.373 {\tiny \color{gray} $\pm$ 0.001} &           1.437 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{33.42} {\tiny \color{gray} $\pm$ 0.08} &           0.086 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\bottomrule
\end{tabular}
}


\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc|ccc|ccc|ccc|ccc|c}
\toprule
     &       & \multicolumn{2}{c}{\;} & \multicolumn{3}{c}{\textsc{ImageNet}} & \multicolumn{3}{c}{\textsc{ImageNet-C (average)}} & \multicolumn{3}{c}{\textsc{ImageNet-A}} & \multicolumn{3}{c}{\textsc{ImageNet-V2}} &                      \textsc{Downstream} \\
     &       & \textsc{K} & \textsc{M} &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ & $\Delta$\textsc{FLOPs} (\%) $\downarrow$ \\
\midrule
\multirow{3}{*}{L/16} & E$^3$ &          2 &          2 &           0.451 {\tiny \color{gray} $\pm$ 0.001} &           12.61 {\tiny \color{gray} $\pm$ 0.04} &           0.023 {\tiny \color{gray} $\pm$ 0.000} &           1.028 {\tiny \color{gray} $\pm$ 0.003} &           24.90 {\tiny \color{gray} $\pm$ 0.07} &           0.028 {\tiny \color{gray} $\pm$ 0.000} &           2.886 {\tiny \color{gray} $\pm$ 0.016} &           58.26 {\tiny \color{gray} $\pm$ 0.24} &           0.171 {\tiny \color{gray} $\pm$ 0.002} &           0.849 {\tiny \color{gray} $\pm$ 0.002} &           21.40 {\tiny \color{gray} $\pm$ 0.11} &           0.055 {\tiny \color{gray} $\pm$ 0.001} &                            \textbf{5.92} \\
     & down-DE &          1 &          4 &  \textbf{0.440} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{12.39} {\tiny \color{gray} $\pm$ 0.06} &  \textbf{0.015} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.983} {\tiny \color{gray} $\pm$ 0.006} &  \textbf{23.95} {\tiny \color{gray} $\pm$ 0.12} &  \textbf{0.020} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{2.712} {\tiny \color{gray} $\pm$ 0.015} &  \textbf{56.36} {\tiny \color{gray} $\pm$ 0.36} &  \textbf{0.120} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{0.803} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{20.83} {\tiny \color{gray} $\pm$ 0.10} &  \textbf{0.039} {\tiny \color{gray} $\pm$ 0.001} &                                   226.53 \\
     & V-MoE &          4 &          1 &           0.465 {\tiny \color{gray} $\pm$ 0.001} &           12.86 {\tiny \color{gray} $\pm$ 0.05} &           0.026 {\tiny \color{gray} $\pm$ 0.000} &           1.060 {\tiny \color{gray} $\pm$ 0.005} &           25.28 {\tiny \color{gray} $\pm$ 0.09} &           0.035 {\tiny \color{gray} $\pm$ 0.000} &           2.976 {\tiny \color{gray} $\pm$ 0.022} &           58.26 {\tiny \color{gray} $\pm$ 0.29} &           0.186 {\tiny \color{gray} $\pm$ 0.002} &           0.856 {\tiny \color{gray} $\pm$ 0.002} &           21.53 {\tiny \color{gray} $\pm$ 0.07} &           0.060 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{L/32} & E$^3$ &          2 &          2 &           0.529 {\tiny \color{gray} $\pm$ 0.001} &           14.63 {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.019} {\tiny \color{gray} $\pm$ 0.000} &           1.188 {\tiny \color{gray} $\pm$ 0.004} &           28.23 {\tiny \color{gray} $\pm$ 0.07} &           0.025 {\tiny \color{gray} $\pm$ 0.000} &           4.095 {\tiny \color{gray} $\pm$ 0.015} &           74.38 {\tiny \color{gray} $\pm$ 0.14} &           0.253 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{0.962} {\tiny \color{gray} $\pm$ 0.001} &           24.41 {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.055} {\tiny \color{gray} $\pm$ 0.001} &                            \textbf{5.54} \\
     & down-DE &          1 &          4 &  \textbf{0.518} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{14.29} {\tiny \color{gray} $\pm$ 0.03} &           0.022 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.154} {\tiny \color{gray} $\pm$ 0.004} &  \textbf{27.47} {\tiny \color{gray} $\pm$ 0.05} &  \textbf{0.023} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{4.033} {\tiny \color{gray} $\pm$ 0.016} &  \textbf{73.79} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{0.237} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{0.959} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{24.03} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.054} {\tiny \color{gray} $\pm$ 0.001} &                                   222.95 \\
     & V-MoE &          4 &          1 &           0.566 {\tiny \color{gray} $\pm$ 0.002} &           15.08 {\tiny \color{gray} $\pm$ 0.04} &           0.041 {\tiny \color{gray} $\pm$ 0.000} &           1.267 {\tiny \color{gray} $\pm$ 0.003} &           29.19 {\tiny \color{gray} $\pm$ 0.05} &           0.053 {\tiny \color{gray} $\pm$ 0.000} &           4.428 {\tiny \color{gray} $\pm$ 0.017} &           75.52 {\tiny \color{gray} $\pm$ 0.06} &           0.306 {\tiny \color{gray} $\pm$ 0.001} &           1.050 {\tiny \color{gray} $\pm$ 0.003} &           25.21 {\tiny \color{gray} $\pm$ 0.05} &           0.084 {\tiny \color{gray} $\pm$ 0.000} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{B/16} & E$^3$ &          2 &          2 &  \textbf{0.510} {\tiny \color{gray} $\pm$ 0.001} &           14.13 {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.016} {\tiny \color{gray} $\pm$ 0.000} &           1.328 {\tiny \color{gray} $\pm$ 0.006} &           30.81 {\tiny \color{gray} $\pm$ 0.11} &  \textbf{0.020} {\tiny \color{gray} $\pm$ 0.000} &           3.743 {\tiny \color{gray} $\pm$ 0.011} &           71.12 {\tiny \color{gray} $\pm$ 0.16} &           0.211 {\tiny \color{gray} $\pm$ 0.002} &           0.945 {\tiny \color{gray} $\pm$ 0.002} &           23.75 {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.044} {\tiny \color{gray} $\pm$ 0.001} &                           \textbf{10.09} \\
     & down-DE &          1 &          4 &  \textbf{0.511} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{13.95} {\tiny \color{gray} $\pm$ 0.01} &           0.019 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.293} {\tiny \color{gray} $\pm$ 0.008} &  \textbf{29.67} {\tiny \color{gray} $\pm$ 0.18} &           0.026 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{3.544} {\tiny \color{gray} $\pm$ 0.015} &  \textbf{66.49} {\tiny \color{gray} $\pm$ 0.27} &  \textbf{0.190} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{0.930} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{23.17} {\tiny \color{gray} $\pm$ 0.06} &           0.050 {\tiny \color{gray} $\pm$ 0.001} &                                   180.41 \\
     & V-MoE &          4 &          1 &           0.532 {\tiny \color{gray} $\pm$ 0.002} &           14.21 {\tiny \color{gray} $\pm$ 0.04} &           0.029 {\tiny \color{gray} $\pm$ 0.001} &           1.350 {\tiny \color{gray} $\pm$ 0.005} &           30.44 {\tiny \color{gray} $\pm$ 0.11} &           0.046 {\tiny \color{gray} $\pm$ 0.001} &           3.726 {\tiny \color{gray} $\pm$ 0.014} &  \textbf{66.88} {\tiny \color{gray} $\pm$ 0.15} &           0.238 {\tiny \color{gray} $\pm$ 0.002} &           0.973 {\tiny \color{gray} $\pm$ 0.003} &           23.69 {\tiny \color{gray} $\pm$ 0.10} &           0.069 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{B/32} & E$^3$ &          2 &          2 &           0.612 {\tiny \color{gray} $\pm$ 0.001} &           16.49 {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.013} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.491} {\tiny \color{gray} $\pm$ 0.003} &           33.85 {\tiny \color{gray} $\pm$ 0.05} &  \textbf{0.019} {\tiny \color{gray} $\pm$ 0.000} &           4.872 {\tiny \color{gray} $\pm$ 0.007} &           82.80 {\tiny \color{gray} $\pm$ 0.08} &  \textbf{0.275} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.099} {\tiny \color{gray} $\pm$ 0.003} &           27.36 {\tiny \color{gray} $\pm$ 0.10} &  \textbf{0.045} {\tiny \color{gray} $\pm$ 0.001} &                            \textbf{9.12} \\
     & down-DE &          1 &          4 &  \textbf{0.607} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{16.17} {\tiny \color{gray} $\pm$ 0.02} &           0.021 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.483} {\tiny \color{gray} $\pm$ 0.008} &  \textbf{33.36} {\tiny \color{gray} $\pm$ 0.13} &           0.027 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{4.787} {\tiny \color{gray} $\pm$ 0.011} &           82.11 {\tiny \color{gray} $\pm$ 0.07} &  \textbf{0.276} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.099} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{26.98} {\tiny \color{gray} $\pm$ 0.01} &           0.055 {\tiny \color{gray} $\pm$ 0.002} &                                   174.26 \\
     & V-MoE &          4 &          1 &           0.636 {\tiny \color{gray} $\pm$ 0.001} &           16.70 {\tiny \color{gray} $\pm$ 0.04} &           0.034 {\tiny \color{gray} $\pm$ 0.001} &           1.555 {\tiny \color{gray} $\pm$ 0.003} &           34.33 {\tiny \color{gray} $\pm$ 0.05} &           0.051 {\tiny \color{gray} $\pm$ 0.001} &           5.031 {\tiny \color{gray} $\pm$ 0.013} &  \textbf{81.62} {\tiny \color{gray} $\pm$ 0.13} &           0.322 {\tiny \color{gray} $\pm$ 0.002} &           1.150 {\tiny \color{gray} $\pm$ 0.003} &           27.49 {\tiny \color{gray} $\pm$ 0.10} &           0.079 {\tiny \color{gray} $\pm$ 0.002} &                                      --- \\
\cmidrule{1-17}
\multirow{3}{*}{S/32} & E$^3$ &          2 &          2 &           0.805 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{20.97} {\tiny \color{gray} $\pm$ 0.05} &  \textbf{0.013} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{2.112} {\tiny \color{gray} $\pm$ 0.007} &           45.05 {\tiny \color{gray} $\pm$ 0.09} &  \textbf{0.028} {\tiny \color{gray} $\pm$ 0.000} &           6.283 {\tiny \color{gray} $\pm$ 0.013} &           93.68 {\tiny \color{gray} $\pm$ 0.09} &           0.342 {\tiny \color{gray} $\pm$ 0.001} &           1.408 {\tiny \color{gray} $\pm$ 0.003} &           33.71 {\tiny \color{gray} $\pm$ 0.10} &  \textbf{0.051} {\tiny \color{gray} $\pm$ 0.001} &                           \textbf{11.70} \\
     & down-DE &          1 &          4 &  \textbf{0.795} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{20.66} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{0.015} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{2.076} {\tiny \color{gray} $\pm$ 0.012} &  \textbf{44.16} {\tiny \color{gray} $\pm$ 0.21} &           0.031 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{5.990} {\tiny \color{gray} $\pm$ 0.011} &           92.25 {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.324} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.372} {\tiny \color{gray} $\pm$ 0.002} &  \textbf{32.83} {\tiny \color{gray} $\pm$ 0.13} &  \textbf{0.054} {\tiny \color{gray} $\pm$ 0.002} &                                   142.29 \\
     & V-MoE &          4 &          1 &           0.820 {\tiny \color{gray} $\pm$ 0.002} &  \textbf{20.97} {\tiny \color{gray} $\pm$ 0.07} &           0.030 {\tiny \color{gray} $\pm$ 0.001} &           2.133 {\tiny \color{gray} $\pm$ 0.006} &  \textbf{44.53} {\tiny \color{gray} $\pm$ 0.12} &           0.060 {\tiny \color{gray} $\pm$ 0.001} &           6.142 {\tiny \color{gray} $\pm$ 0.014} &  \textbf{91.62} {\tiny \color{gray} $\pm$ 0.12} &           0.365 {\tiny \color{gray} $\pm$ 0.002} &           1.417 {\tiny \color{gray} $\pm$ 0.003} &  \textbf{33.30} {\tiny \color{gray} $\pm$ 0.12} &           0.081 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\bottomrule
\end{tabular}
}


\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc|ccc|ccc|c}
\toprule
     &       & \multicolumn{2}{c}{\;} & \multicolumn{3}{c}{\textsc{Cifar10}} & \multicolumn{3}{c}{\textsc{Cifar10-C}} &                      \textsc{Downstream} \\
     &       & \textsc{K} & \textsc{M} &                        \textsc{NLL} $\downarrow$ &                    \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ & $\Delta$\textsc{FLOPs} (\%) $\downarrow$ \\
\midrule
\multirow{3}{*}{L/16} & E$^3$ &          1 &          2 &  \textbf{0.022} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.55} {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.198} {\tiny \color{gray} $\pm$ 0.012} &   \textbf{5.65} {\tiny \color{gray} $\pm$ 0.20} &  \textbf{0.027} {\tiny \color{gray} $\pm$ 0.002} &                            \textbf{6.74} \\
     & down-DE &          1 &          2 &           0.026 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.59} {\tiny \color{gray} $\pm$ 0.04} &           0.004 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.227} {\tiny \color{gray} $\pm$ 0.011} &   \textbf{6.18} {\tiny \color{gray} $\pm$ 0.21} &  \textbf{0.032} {\tiny \color{gray} $\pm$ 0.003} &                                    86.04 \\
     & V-MoE &          2 &          1 &           0.028 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.61} {\tiny \color{gray} $\pm$ 0.01} &           0.004 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.220} {\tiny \color{gray} $\pm$ 0.012} &   \textbf{6.17} {\tiny \color{gray} $\pm$ 0.23} &  \textbf{0.032} {\tiny \color{gray} $\pm$ 0.003} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{L/32} & E$^3$ &          1 &          2 &  \textbf{0.026} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.69} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.246} {\tiny \color{gray} $\pm$ 0.008} &   \textbf{7.01} {\tiny \color{gray} $\pm$ 0.15} &  \textbf{0.033} {\tiny \color{gray} $\pm$ 0.002} &                            \textbf{6.35} \\
     & down-DE &          1 &          2 &           0.034 {\tiny \color{gray} $\pm$ 0.001} &           0.81 {\tiny \color{gray} $\pm$ 0.02} &           0.005 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.252} {\tiny \color{gray} $\pm$ 0.013} &   \textbf{7.00} {\tiny \color{gray} $\pm$ 0.26} &  \textbf{0.032} {\tiny \color{gray} $\pm$ 0.004} &                                    85.29 \\
     & V-MoE &          2 &          1 &           0.042 {\tiny \color{gray} $\pm$ 0.001} &           0.90 {\tiny \color{gray} $\pm$ 0.03} &           0.006 {\tiny \color{gray} $\pm$ 0.000} &           0.325 {\tiny \color{gray} $\pm$ 0.011} &            8.05 {\tiny \color{gray} $\pm$ 0.17} &           0.048 {\tiny \color{gray} $\pm$ 0.002} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{B/16} & E$^3$ &          1 &          2 &           0.036 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.84} {\tiny \color{gray} $\pm$ 0.02} &           0.005 {\tiny \color{gray} $\pm$ 0.000} &           0.295 {\tiny \color{gray} $\pm$ 0.008} &            8.28 {\tiny \color{gray} $\pm$ 0.15} &           0.038 {\tiny \color{gray} $\pm$ 0.002} &                           \textbf{12.60} \\
     & down-DE &          1 &          2 &  \textbf{0.030} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.81} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.247} {\tiny \color{gray} $\pm$ 0.005} &   \textbf{7.60} {\tiny \color{gray} $\pm$ 0.16} &  \textbf{0.028} {\tiny \color{gray} $\pm$ 0.001} &                                    75.09 \\
     & V-MoE &          2 &          1 &           0.040 {\tiny \color{gray} $\pm$ 0.001} &           0.97 {\tiny \color{gray} $\pm$ 0.02} &           0.006 {\tiny \color{gray} $\pm$ 0.000} &           0.303 {\tiny \color{gray} $\pm$ 0.008} &   \textbf{8.08} {\tiny \color{gray} $\pm$ 0.09} &           0.047 {\tiny \color{gray} $\pm$ 0.002} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{B/32} & E$^3$ &          1 &          2 &           0.041 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.11} {\tiny \color{gray} $\pm$ 0.03} &           0.004 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.340} {\tiny \color{gray} $\pm$ 0.010} &  \textbf{10.01} {\tiny \color{gray} $\pm$ 0.18} &  \textbf{0.040} {\tiny \color{gray} $\pm$ 0.003} &                           \textbf{11.54} \\
     & down-DE &          1 &          2 &  \textbf{0.036} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{1.07} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.345} {\tiny \color{gray} $\pm$ 0.006} &           10.87 {\tiny \color{gray} $\pm$ 0.13} &  \textbf{0.042} {\tiny \color{gray} $\pm$ 0.002} &                                    73.49 \\
     & V-MoE &          2 &          1 &           0.042 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.11} {\tiny \color{gray} $\pm$ 0.03} &           0.006 {\tiny \color{gray} $\pm$ 0.000} &           0.405 {\tiny \color{gray} $\pm$ 0.015} &           11.30 {\tiny \color{gray} $\pm$ 0.24} &           0.063 {\tiny \color{gray} $\pm$ 0.004} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{S/32} & E$^3$ &          1 &          2 &           0.060 {\tiny \color{gray} $\pm$ 0.001} &           1.92 {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.476} {\tiny \color{gray} $\pm$ 0.007} &  \textbf{15.30} {\tiny \color{gray} $\pm$ 0.17} &  \textbf{0.049} {\tiny \color{gray} $\pm$ 0.002} &                           \textbf{15.86} \\
     & down-DE &          1 &          2 &  \textbf{0.056} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.75} {\tiny \color{gray} $\pm$ 0.03} &           0.005 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.491} {\tiny \color{gray} $\pm$ 0.004} &  \textbf{15.42} {\tiny \color{gray} $\pm$ 0.15} &           0.064 {\tiny \color{gray} $\pm$ 0.001} &                                    64.34 \\
     & V-MoE &          2 &          1 &  \textbf{0.058} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.80} {\tiny \color{gray} $\pm$ 0.03} &           0.007 {\tiny \color{gray} $\pm$ 0.000} &           0.514 {\tiny \color{gray} $\pm$ 0.006} &  \textbf{15.48} {\tiny \color{gray} $\pm$ 0.21} &           0.076 {\tiny \color{gray} $\pm$ 0.002} &                                      --- \\
\bottomrule
\end{tabular}
}


\resizebox{\linewidth}{!}{
\begin{tabular}{cc|cc|ccc|ccc|c}
\toprule
     &       & \multicolumn{2}{c}{\;} & \multicolumn{3}{c}{\textsc{Cifar10}} & \multicolumn{3}{c}{\textsc{Cifar10-C}} &                      \textsc{Downstream} \\
     &       & \textsc{K} & \textsc{M} &                        \textsc{NLL} $\downarrow$ &                    \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ &                        \textsc{NLL} $\downarrow$ &                     \textsc{Error} $\downarrow$ &                        \textsc{ECE} $\downarrow$ & $\Delta$\textsc{FLOPs} (\%) $\downarrow$ \\
\midrule
\multirow{3}{*}{L/16} & E$^3$ &          2 &          2 &  \textbf{0.026} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.58} {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.247} {\tiny \color{gray} $\pm$ 0.016} &   \textbf{6.56} {\tiny \color{gray} $\pm$ 0.26} &  \textbf{0.036} {\tiny \color{gray} $\pm$ 0.003} &                            \textbf{5.92} \\
     & down-DE &          1 &          4 &  \textbf{0.025} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.57} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.004} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.219} {\tiny \color{gray} $\pm$ 0.010} &   \textbf{6.12} {\tiny \color{gray} $\pm$ 0.19} &  \textbf{0.030} {\tiny \color{gray} $\pm$ 0.003} &                                   226.53 \\
     & V-MoE &          4 &          1 &           0.034 {\tiny \color{gray} $\pm$ 0.001} &           0.75 {\tiny \color{gray} $\pm$ 0.02} &           0.005 {\tiny \color{gray} $\pm$ 0.000} &           0.278 {\tiny \color{gray} $\pm$ 0.010} &            7.71 {\tiny \color{gray} $\pm$ 0.19} &           0.043 {\tiny \color{gray} $\pm$ 0.002} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{L/32} & E$^3$ &          2 &          2 &  \textbf{0.033} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.80} {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.004} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.242} {\tiny \color{gray} $\pm$ 0.006} &   \textbf{6.65} {\tiny \color{gray} $\pm$ 0.12} &  \textbf{0.031} {\tiny \color{gray} $\pm$ 0.002} &                            \textbf{5.54} \\
     & down-DE &          1 &          4 &  \textbf{0.030} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.78} {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.004} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.232} {\tiny \color{gray} $\pm$ 0.012} &   \textbf{6.74} {\tiny \color{gray} $\pm$ 0.27} &  \textbf{0.028} {\tiny \color{gray} $\pm$ 0.003} &                                   222.94 \\
     & V-MoE &          4 &          1 &           0.035 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.81} {\tiny \color{gray} $\pm$ 0.02} &           0.005 {\tiny \color{gray} $\pm$ 0.000} &           0.295 {\tiny \color{gray} $\pm$ 0.009} &            7.63 {\tiny \color{gray} $\pm$ 0.14} &           0.044 {\tiny \color{gray} $\pm$ 0.002} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{B/16} & E$^3$ &          2 &          2 &           0.034 {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.81} {\tiny \color{gray} $\pm$ 0.02} &           0.004 {\tiny \color{gray} $\pm$ 0.000} &           0.283 {\tiny \color{gray} $\pm$ 0.006} &            8.06 {\tiny \color{gray} $\pm$ 0.12} &           0.037 {\tiny \color{gray} $\pm$ 0.002} &                           \textbf{10.09} \\
     & down-DE &          1 &          4 &  \textbf{0.029} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.80} {\tiny \color{gray} $\pm$ 0.03} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.242} {\tiny \color{gray} $\pm$ 0.006} &   \textbf{7.54} {\tiny \color{gray} $\pm$ 0.16} &  \textbf{0.026} {\tiny \color{gray} $\pm$ 0.001} &                                   180.41 \\
     & V-MoE &          4 &          1 &  \textbf{0.032} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{0.79} {\tiny \color{gray} $\pm$ 0.02} &           0.005 {\tiny \color{gray} $\pm$ 0.000} &           0.266 {\tiny \color{gray} $\pm$ 0.004} &   \textbf{7.55} {\tiny \color{gray} $\pm$ 0.10} &           0.040 {\tiny \color{gray} $\pm$ 0.001} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{B/32} & E$^3$ &          2 &          2 &  \textbf{0.034} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.00} {\tiny \color{gray} $\pm$ 0.02} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.306} {\tiny \color{gray} $\pm$ 0.009} &   \textbf{9.44} {\tiny \color{gray} $\pm$ 0.23} &  \textbf{0.037} {\tiny \color{gray} $\pm$ 0.002} &                            \textbf{9.12} \\
     & down-DE &          1 &          4 &  \textbf{0.035} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.06} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.003} {\tiny \color{gray} $\pm$ 0.000} &           0.338 {\tiny \color{gray} $\pm$ 0.005} &           10.77 {\tiny \color{gray} $\pm$ 0.12} &  \textbf{0.040} {\tiny \color{gray} $\pm$ 0.002} &                                   174.26 \\
     & V-MoE &          4 &          1 &           0.042 {\tiny \color{gray} $\pm$ 0.001} &           1.12 {\tiny \color{gray} $\pm$ 0.02} &           0.006 {\tiny \color{gray} $\pm$ 0.000} &           0.410 {\tiny \color{gray} $\pm$ 0.017} &           11.29 {\tiny \color{gray} $\pm$ 0.26} &           0.066 {\tiny \color{gray} $\pm$ 0.004} &                                      --- \\
\cmidrule{1-11}
\multirow{3}{*}{S/32} & E$^3$ &          2 &          2 &           0.058 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.82} {\tiny \color{gray} $\pm$ 0.01} &  \textbf{0.004} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.472} {\tiny \color{gray} $\pm$ 0.007} &  \textbf{15.01} {\tiny \color{gray} $\pm$ 0.17} &  \textbf{0.051} {\tiny \color{gray} $\pm$ 0.002} &                           \textbf{11.69} \\
     & down-DE &          1 &          4 &  \textbf{0.055} {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.76} {\tiny \color{gray} $\pm$ 0.04} &  \textbf{0.004} {\tiny \color{gray} $\pm$ 0.000} &  \textbf{0.486} {\tiny \color{gray} $\pm$ 0.003} &  \textbf{15.36} {\tiny \color{gray} $\pm$ 0.13} &           0.061 {\tiny \color{gray} $\pm$ 0.001} &                                   142.28 \\
     & V-MoE &          4 &          1 &           0.059 {\tiny \color{gray} $\pm$ 0.001} &  \textbf{1.80} {\tiny \color{gray} $\pm$ 0.05} &           0.007 {\tiny \color{gray} $\pm$ 0.000} &           0.536 {\tiny \color{gray} $\pm$ 0.012} &  \textbf{15.64} {\tiny \color{gray} $\pm$ 0.27} &           0.084 {\tiny \color{gray} $\pm$ 0.004} &                                      --- \\
\bottomrule
\end{tabular}
}
